Beyond Polarization: The Generative Constraint of Chain-of-Thought in Pointwise Reranking

In pointwise document reranking, Chain-of-Thought models typically underperform direct scoring models. While existing diagnostics attribute this to inferior classification, score polarization, or calibration breakdown, whether targeted training can bridge this gap remains unclear. Our empirical study first confirms that this gap is stable across scales up to 32B parameters, ruling out model and data capacity confounders. We then apply stress tests utilizing reinforcement learning, fine-grained supervision, and architectural decoupling to explicitly repair these deviations. Although these interventions improve classification accuracy and absolute scores, the relative ranking gap persists. These findings suggest that, within the pointwise scoring paradigm, routing continuous relevance semantics through discrete text constrains ranking signal resolution, revealing a bottleneck that is stable and difficult to overcome under current standard methods, rather than an easily resolvable training bias.

==> latex/test.tex <==
\section{StageII: Stress Tests on the Performance Gap}
\label{sec:stage2}

In this section, we further ask: \textit{Can targeted interventions addressing known deviations truly bridge the gap?} To answer this, we conduct three stress tests on the Qwen3 series targeting inferior classification accuracy, score polarization, and probability calibration breakdown. Results across the three benchmarks are summarized in Table~\ref{tab:stage2}.

\subsection{Reinforcement Learning Alignment}
\label{sec:rl}

Targeting inferior classification accuracy, we apply GRPO to SFT CoT to test whether explicitly aligning the classification boundary with Direct Scoring restores ranking performance. 

Given a generation $y$ and a binary label $g\!\in\!\{\textsc{true},\textsc{false}\}$, we integrate structural constraints as a gating function $\mathbf{1}[\text{valid}]$ (requiring paired \texttt{<think>...</think>} tags followed by an \texttt{Answer:\,<true|false>} pattern) directly into the reward function:
\begin{equation} \resizebox{0.95\linewidth}{!}{$ R(y,g) = \mathbf{1}[\text{valid}] \cdot \big( \alpha\mathbf{1}[\text{thk}] + \beta\mathbf{1}[\text{fmt}] + \gamma\mathbf{1}[\text{match}] \big) $} \end{equation} 
When valid, the reward is a weighted sum of lightweight formatting terms (structural validity $\alpha\!=\!0.1$, answer format $\beta\!=\!0.1$) and classification correctness which dominates the gradient ($\gamma\!=\!0.8$ only when the parsed label matches $g$). This design maintains output protocols while fully aligning the RL signal with the binary classification objective of Direct Scoring, allowing us to test: \textit{Does the ranking gap persist when both share the same classification boundary?}

As shown in Figure~\ref{fig:grpo_cls}, GRPO \textbf{matches or even surpasses} the classification accuracy of noCoT in 8 out of 9 evaluation units (scale $\times$ dataset), falling marginally short by 0.1\,pt only on BRIGHT of Qwen3-14B. This alignment holds across other scales. However, the corresponding NDCG@10 gap does not close synchronously: although the deficit for 14B on DL19 narrows from $-3.1$ to $-0.3$, noCoT still maintains a lead of 0.3 to 3.7 across all units. \textit{Aligning classification boundaries does not fully translate into ranking quality, indicating a divergence between classification accuracy and ranking performance.}

\subsection{Fine-Grained Supervision}
\label{sec:mtag}

Targeting score polarization, we train \textbf{Mtag-noCoT} and \textbf{Mtag-CoT} using Gemini-3-Pro distilled data to test whether denser supervision improves the discrimination of partially relevant documents. After the \texttt{Answer:} prompt, both variants simultaneously output binary and fine-grained 0 to 4 scores, with the final relevance derived from a weighted sum of both logits. Results show that Mtag-noCoT achieves the optimal performance. While Mtag-CoT improves significantly over standard Gemini CoT, it still lags behind Mtag-noCoT by 3.3 to 11.3 NDCG. \textit{Fine-grained supervision synchronously raises the performance ceiling for both paradigms, failing to narrow the relative gap.}

\subsection{Architectural Decoupling}
\label{sec:decouple}

Targeting probability calibration breakdown caused by computational coupling within a single decoding pass, we design an explicit two-stage cascade to test whether severing this entanglement resolves the ranking deficit. A generator $M_{g}$ first emits a rationale $t$, which is then concatenated with the original input and fed to a separate scorer $M_{s}$ that outputs only the score token. This severs all computational coupling between reasoning and scoring while preserving the same training data and supervision. As shown in Table~\ref{tab:stage2}, \textbf{+Decouple} narrows the gap relative to standard CoT in most units, for instance from $-11.3$ to $-3.6$ on DL19-0.6B, indicating that computational coupling does account for a non-trivial portion of the deficit. Yet noCoT continues to lead by 0.4 to 7.9 NDCG across all 9 units, and on DL20-8B the gap even widens slightly from $-7.1$ to $-7.9$. \textit{Decoupling computation alleviates but does not eliminate the deficit; a residual gap remains because both stages still route their decision through the discrete reasoning trace $t$.}

